TopoLoRA-SAM: Topology-Aware Parameter-Efficient Adaptation of Foundation Segmenters for Thin-Structure and Cross-Domain Binary Semantic Segmentation

Foundation segmentation models such as the Segment Anything Model (SAM) exhibit strong zero-shot generalization through large-scale pretraining, but adapting them to domain-specific semantic segmentation remains challenging, particularly for thin structures (e.g., retinal vessels) and noisy modalities (e.g., SAR imagery). Full fine-tuning is computationally expensive and risks catastrophic forgetting. We propose \textbf{TopoLoRA-SAM}, a topology-aware and parameter-efficient adaptation framework for binary semantic segmentation. TopoLoRA-SAM injects Low-Rank Adaptation (LoRA) into the frozen ViT encoder, augmented with a lightweight spatial convolutional adapter and optional topology-aware supervision via differentiable clDice. We evaluate our approach on five benchmarks spanning retinal vessel segmentation (DRIVE, STARE, CHASE\_DB1), polyp segmentation (Kvasir-SEG), and SAR sea/land segmentation (SL-SSDD), comparing against U-Net, DeepLabV3+, SegFormer, and Mask2Former. TopoLoRA-SAM achieves the best retina-average Dice and the best overall average Dice across datasets, while training only \textbf{5.2\%} of model parameters ($\sim$4.9M). On the challenging CHASE\_DB1 dataset, our method substantially improves segmentation accuracy and robustness, demonstrating that topology-aware parameter-efficient adaptation can match or exceed fully fine-tuned specialist models. Code is available at : https://github.com/salimkhazem/Seglab.git

==> ICPR_2026_LaTeX_Templates/tables_icpr/paper_bfscore_retina.tex <==
\begin{tabular}{llllll}
\toprule
 & U-Net (R34) & DeepLabV3+ (R50) & SegFormer (B0) & Mask2Former (Swin-T) & TopoLoRA-SAM (ours) \\
\midrule
DRIVE & 0.504±0.140 & 0.466±0.028 & 0.360±0.079 & \textbf{0.746±0.011} & 0.688±0.030 \\
STARE & 0.318±0.091 & 0.320±0.036 & 0.169±0.008 & \textbf{0.662±0.011} & 0.572±0.059 \\
CHASE\_DB1 & 0.260±0.037 & 0.214±0.050 & 0.208±0.013 & 0.194±0.337 & \textbf{0.473±0.050} \\
Retina Avg & 0.361±0.140 & 0.333±0.115 & 0.246±0.096 & 0.534±0.308 & \textbf{0.578±0.102} \\
\bottomrule
\end{tabular}


==> ICPR_2026_LaTeX_Templates/tables_icpr/paper_cldice_retina.tex <==
\begin{tabular}{llllll}
\toprule
 & U-Net (R34) & DeepLabV3+ (R50) & SegFormer (B0) & Mask2Former (Swin-T) & TopoLoRA-SAM (ours) \\
\midrule
DRIVE & 0.609±0.063 & 0.622±0.019 & 0.510±0.043 & 0.673±0.019 & \textbf{0.678±0.021} \\
STARE & 0.417±0.163 & 0.520±0.062 & 0.316±0.015 & \textbf{0.630±0.047} & 0.560±0.052 \\
CHASE\_DB1 & 0.397±0.089 & 0.428±0.119 & 0.391±0.031 & 0.534±0.046 & \textbf{0.599±0.014} \\
Retina Avg & 0.474±0.141 & 0.524±0.108 & 0.406±0.089 & 0.612±0.071 & \textbf{0.612±0.060} \\
\bottomrule
\end{tabular}


==> ICPR_2026_LaTeX_Templates/tables_icpr/paper_ece.tex <==
\begin{tabular}{llllll}
\toprule
 & U-Net (R34) & DeepLabV3+ (R50) & SegFormer (B0) & Mask2Former (Swin-T) & TopoLoRA-SAM (ours) \\
\midrule
DRIVE & 0.204±0.079 & 0.108±0.012 & 0.037±0.009 & \textbf{0.028±0.003} & 0.043±0.009 \\
STARE & 0.291±0.094 & 0.188±0.015 & \textbf{0.028±0.002} & 0.031±0.003 & 0.042±0.010 \\
CHASE\_DB1 & 0.262±0.085 & 0.224±0.092 & 0.055±0.012 & 0.635±0.526 & \textbf{0.045±0.009} \\
Kvasir-SEG & 0.022±0.004 & 0.026±0.006 & 0.023±0.001 & \textbf{0.017±0.003} & 0.026±0.005 \\
SL-SSDD & 0.005±0.002 & 0.004±0.000 & 0.003±0.001 & 0.006±0.001 & \textbf{0.003±0.001} \\
Retina Avg & 0.253±0.084 & 0.173±0.070 & \textbf{0.040±0.014} & 0.232±0.401 & 0.043±0.008 \\
Overall Avg & 0.157±0.137 & 0.110±0.096 & \textbf{0.029±0.019} & 0.144±0.323 & 0.031±0.018 \\
\bottomrule
\end{tabular}


==> tables_icpr/paper_bfscore_retina.tex <==
\begin{tabular}{llllll}
\toprule
 & U-Net (R34) & DeepLabV3+ (R50) & SegFormer (B0) & Mask2Former (Swin-T) & TopoLoRA-SAM (ours) \\
\midrule
DRIVE & 0.504±0.140 & 0.466±0.028 & 0.360±0.079 & \textbf{0.746±0.011} & 0.688±0.030 \\
STARE & 0.318±0.091 & 0.320±0.036 & 0.169±0.008 & \textbf{0.662±0.011} & 0.572±0.059 \\
CHASE\_DB1 & 0.260±0.037 & 0.214±0.050 & 0.208±0.013 & 0.194±0.337 & \textbf{0.473±0.050} \\
Retina Avg & 0.361±0.140 & 0.333±0.115 & 0.246±0.096 & 0.534±0.308 & \textbf{0.578±0.102} \\
\bottomrule
\end{tabular}


==> tables_icpr/paper_cldice_retina.tex <==
\begin{tabular}{llllll}
\toprule
 & U-Net (R34) & DeepLabV3+ (R50) & SegFormer (B0) & Mask2Former (Swin-T) & TopoLoRA-SAM (ours) \\
\midrule
DRIVE & 0.609±0.063 & 0.622±0.019 & 0.510±0.043 & 0.673±0.019 & \textbf{0.678±0.021} \\
STARE & 0.417±0.163 & 0.520±0.062 & 0.316±0.015 & \textbf{0.630±0.047} & 0.560±0.052 \\
CHASE\_DB1 & 0.397±0.089 & 0.428±0.119 & 0.391±0.031 & 0.534±0.046 & \textbf{0.599±0.014} \\
Retina Avg & 0.474±0.141 & 0.524±0.108 & 0.406±0.089 & 0.612±0.071 & \textbf{0.612±0.060} \\
\bottomrule
\end{tabular}


==> tables_icpr/paper_dice.tex <==
\begin{tabular}{llllll}
\toprule
 & U-Net (R34) & DeepLabV3+ (R50) & SegFormer (B0) & Mask2Former (Swin-T) & TopoLoRA-SAM (ours) \\
\midrule
DRIVE & 0.590±0.059 & 0.589±0.027 & 0.541±0.041 & 0.689±0.011 & \textbf{0.690±0.018} \\
STARE & 0.433±0.131 & 0.478±0.056 & 0.374±0.016 & \textbf{0.644±0.023} & 0.565±0.048 \\
CHASE\_DB1 & 0.412±0.050 & 0.345±0.123 & 0.424±0.011 & 0.285±0.293 & \textbf{0.569±0.016} \\
Kvasir-SEG & 0.922±0.004 & 0.917±0.003 & 0.920±0.005 & \textbf{0.933±0.012} & 0.930±0.002 \\
SL-SSDD & 0.993±0.001 & 0.993±0.000 & 0.994±0.000 & 0.992±0.001 & \textbf{0.994±0.000} \\
Retina Avg & 0.478±0.113 & 0.470±0.126 & 0.446±0.077 & 0.539±0.242 & \textbf{0.595±0.049} \\
Overall Avg & 0.670±0.259 & 0.664±0.265 & 0.650±0.267 & 0.709±0.283 & \textbf{0.735±0.185} \\
\bottomrule
\end{tabular}


==> tables_icpr/paper_ece.tex <==
\begin{tabular}{llllll}
\toprule
 & U-Net (R34) & DeepLabV3+ (R50) & SegFormer (B0) & Mask2Former (Swin-T) & TopoLoRA-SAM (ours) \\
\midrule
DRIVE & 0.204±0.079 & 0.108±0.012 & 0.037±0.009 & \textbf{0.028±0.003} & 0.043±0.009 \\
STARE & 0.291±0.094 & 0.188±0.015 & \textbf{0.028±0.002} & 0.031±0.003 & 0.042±0.010 \\
CHASE\_DB1 & 0.262±0.085 & 0.224±0.092 & 0.055±0.012 & 0.635±0.526 & \textbf{0.045±0.009} \\
Kvasir-SEG & 0.022±0.004 & 0.026±0.006 & 0.023±0.001 & \textbf{0.017±0.003} & 0.026±0.005 \\
SL-SSDD & 0.005±0.002 & 0.004±0.000 & 0.003±0.001 & 0.006±0.001 & \textbf{0.003±0.001} \\
Retina Avg & 0.253±0.084 & 0.173±0.070 & \textbf{0.040±0.014} & 0.232±0.401 & 0.043±0.008 \\
Overall Avg & 0.157±0.137 & 0.110±0.096 & \textbf{0.029±0.019} & 0.144±0.323 & 0.031±0.018 \\
\bottomrule
\end{tabular}

